Bayesian Optimization Meets Self-Distillation

Bayesian optimization (BO) has contributed greatly to improving model performance by suggesting promising hyperparameter configurations iteratively based on observations from multiple training trials. However, only partial knowledge (i.e., the measured performances of trained models and their hyperparameter configurations) from previous trials is transferred. On the other hand, Self-Distillation (SD) only transfers partial knowledge learned by the task model itself. To fully leverage the various knowledge gained from all training trials, we propose the BOSS framework, which combines BO and SD. BOSS suggests promising hyperparameter configurations through BO and carefully selects pre-trained models from previous trials for SD, which are otherwise abandoned in the conventional BO process. BOSS achieves significantly better performance than both BO and SD in a wide range of tasks including general image classification, learning with noisy labels, semi-supervised learning, and medical image analysis tasks.

==> 0.abstract.tex <==
\begin{abstract}
The performance of modern Convolutional Neural Networks (CNNs) is highly dependent on the choice of hyperparameters. Recently, Bayesian optimization (BO) has emerged as a popular method for hyperparameter optimization. It adaptively suggests promising hyperparameter configurations based on the observations that come from the previous configurations. However, BO does not utilize the knowledge acquired by CNNs for further improvements, which has been shown to contain valuable information in recent studies of self-distillation (SD). In order to fully leverage the potential of this knowledge, we propose \ours which combines SD into the BO process. The proposed method transfers knowledge learned in former trials to latter trials via SD, enhancing the performance of CNNs. It achieves remarkable performance improvements in a wide range of tasks including general image classification, learning with noisy labels, semi-supervised learning, and medical image analysis tasks. 
\end{abstract}

==> 1.introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\begin{figure*}
\begin{center}
    \includegraphics[width=0.95\textwidth]{figure/method.pdf}
    \caption{Illustration of the proposed method, \ours. For each iteration, Bayesian optimization suggests the next configuration evaluation based on the previous observations. After that, the knowledge learned by the network in previous trials is utilized for training the next network with a form of self-distillation.
    \swp{\ours is a novel framework for training models, which fuses the Bayesian Optimization (BO) and Self-Distillation (SD), combining the concept of hyperparameter exploration and knowledge distillation. By performing these steps simply in an alternating manner (left-to-right), we propagate both the conditional probability learned over hyperparameter configurations (depicted with graphs) and the knowledge learned by each task network, resulting in large performance gains in the final model.}
    \swp{This figure needs to be referenced via \autoref{fig:method}}
    }
    \label{fig:method}
\end{center}
\vspace{-8mm}
\end{figure*}

Convolutional Neural Networks (CNNs) have achieved remarkable success in a wide range of computer vision applications \cite{chen2017deeplab, lee2019srm, liu2016ssd}. However, their performance is greatly dependent on the choice of hyperparameters \cite{choi2019empirical}. As the optimal hyperparameter configuration is not known a priori, practitioners often explore the hyperparameter space manually to obtain a better configuration. Despite its time-consuming process, it typically results in sub-optimal performance \cite{bergstra2012random}.
Recently, Bayesian optimization (BO) has emerged as a successful approach to hyperparameter optimization, automating the manual tuning effort and pushing the boundaries of performance \cite{bergstra2011algorithms,hutter2011sequential,snoek2012practical}. BO allows for the effective exploration of multi-dimensional search spaces by suggesting promising configurations based on observations. This technique has achieved state-of-the-art performance for training CNNs \cite{bergstra2013making, falkner2018bohb} and has contributed to improving various applications such as AlphaGo \cite{chen2018bayesian}. 

BO is inherently an iterative process in which a probabilistic prior model is fitted using observations of hyperparameter configurations and their corresponding performances \cite{bergstra2011algorithms, hutter2011sequential}. At each iteration, BO suggests the next configuration to evaluate that is most likely to improve performance. After training the network with the suggested configuration, a new observation is retrieved and used to update the probabilistic model. 
However, despite BO's adaptive use of observed configurations and their corresponding performances, it discards the past knowledge learned by the network.
\swp{Discard? Or Forget? The last statement also seems a bit sudden. Can you be more explicit: it does not propagate knowledge learned in the early stages to the late stages very well.}

A recent line of research in self-distillation (SD) has demonstrated that transferring knowledge from a previously trained model with the identical capacity can improve the performance of the model \cite{allen2020towards, furlanello2018born, pham2022revisiting}.
If a student network is trained to mimic the feature distribution of a teacher network, then the student could beat the teacher.
Allen-Zhu and Li \cite{allen2020towards} have both theoretically and empirically interpreted this as a similar effect to ensembling various models. Inspired by these studies and the iterative nature of BO, we ended up asking if the network's knowledge from the previous trials could be used for the next trials to reach a higher performance of the target task.

In this paper, we propose \textit{Hyperparameter Optimization via Bayesian Optimization and Self-Distillation for Effective Knowledge Transfer} (\ours) which integrates SD into the BO process to fully leverage the knowledge learned in previous trials. 
The overall process of \ours is illustrated in Figure~\ref{fig:method}. 
Following the BO process, \ours suggests a hyperparameter configuration based on observations that are most likely to improve the performance. 
Additionally, it transfers past knowledge by conveying the network trained during previous trials and then training the network with SD.
This process is performed in an iterative manner, allowing the network to persistently improve upon previous trials.
%by utilizing prior knowledge as a stepping stone to push the boundaries of performance. 
To the best of our knowledge, this is the first work that leverages the knowledge of the network learned during BO process. \dg{This is not a simple combination of two orthogonal methods but we propose an optimal solution to the problem of how to transfer past knowledge.}
\swp{``Optimal Solution'' can easily trigger some reviewers if you don't provide a theoretical guarantee, I would be cautious.}
%, which is backed by our rigorous experiments.}
\dgdg{The suggested solution is that (1) both the student and the teacher should be initialized from prior knowledge, and that (2) they should be differently initialized from different previous trials to fully exploit the prior knowledge. Our thorough ablation analysis supports this.}
%\hs{A significant aspect of our approach is the careful design of pre-trained weight selection not only for the teacher but also for the student, which enables}
%\hj{to fully exploit the potential of the past knowledge.}
%\hs{Our experiments show that the selection design significantly impacts model performance. Furthermore, the simplicity and effectiveness of our approach enable its generalization to various CNN structures and BO methods.}

We evaluate the effectiveness of \ours \dg{with} various computer vision tasks, such as object classification~\cite{he2016deep}, learning with noisy labels~\cite{han2018co}, and semi-supervised learning~\cite{arazo2020pseudo}. In addition, we also evaluate it \dg{with} medical image analysis tasks, including medical image segmentation and classification. Our experimental results demonstrate that \ours significantly improves \swp{target} model performance  without introducing any additional overhead at test time. Furthermore, we conduct comprehensive analysis and ablation studies to further investigate the behavior of \ours. 
%\dg{Finally,} our experiments show that \ours is applicable to a variety of BO and SD methods, demonstrating its practicality across a wide range of scenarios.

In summary, the main contributions of this paper are:
\begin{inparaenum}[i)]
% \begin{itemize}
  \item we present \hs{HypeBOSS} which enhances Bayesian optimization (BO) by exploiting the knowledge of the network learned during BO process,
  \item our proposed method yields significant performance improvements in various tasks without introducing any additional overhead at test time, and
  \item through extensive analysis and ablation studies, we examine the validity of our method and demonstrate its practicality across a wide range of scenarios.
% \end{itemize}
\end{inparaenum}



==> 2.related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\swp{This entire section is so verbose, but why? Can't it be much shorter? This section should keep the reader engaged w.r.t. your contributions, not bore them with the history.}

\parahead{Bayesian Optimization}
Bayesian optimization (BO) is a global optimization method 
for black-box functions \cite{bergstra2011algorithms}. 
%with no available closed-form expressions or derivatives 
%BO is widely adopted for hyperparameter optimization due to its ability to efficiently optimize expensive functions \cite{hutter2019automated}.
Given a set of hyperparameters $\lambda$ and an objective function $\Phi$ (e.g. accuracy), BO models the conditional probability $p(\Phi(\lambda)|\lambda)$ with a surrogate model. 
In each iteration, it fits the surrogate model given observations then uses the acquisition function to determine which configuration to evaluate next. 
By suggesting probable candidates based on observations, it has shown remarkable performance on various hyperparameter optimization tasks \cite{bergstra2011algorithms,hutter2011sequential,snoek2012practical}. 

Gaussian Process (GP) \cite{rasmussen2006gaussian} is a popular surrogate model due to its smoothness and well-calibrated uncertainty estimates. However, its computational cost grows cubically with the number of observations, making it less suitable for high-dimensional search spaces. 
%Moreover, its kernel function needs to be chosen carefully for different tasks. 
Sequential Model-based Algorithm Configuration (SMAC) \cite{hutter2011sequential} is an alternative model that uses random forests to model $p(\Phi(\lambda)|\lambda)$. It has a computational complexity of $O(n \log n)$ and can handle categorical and conditional search spaces more effectively than GP. Instead of modeling $p(\Phi(\lambda)|\lambda)$, the Tree-structured Parzen Estimator (TPE) \cite{bergstra2011algorithms} models $p(\lambda|\Phi(\lambda))$ \hj{by partitioning hyperparameter density function into good and bad groups with respect to their corresponding objective values}. It has linear complexity on the number of observations and enables scalable hyperparameter optimization.

There have been various approaches to improve BO by incorporating prior knowledge. A line of works aims to transfer knowledge learned from other datasets through meta-learning. Multi-objective TPE \cite{watanabe2022multi} extends TPE to transfer knowledge from other tasks considering the similarity between tasks. Surrogate-Based Collaborative Tuning \cite{bardenet2013collaborative} leverages the knowledge from various datasets by integrating the surrogate ranking algorithm into BO.
On the other hand, Prior-guided Bayesian Optimization \cite{souza2020prior} allows domain experts to transfer their knowledge into BO in the form of priors.
%, which results in faster convergence compared to standard BO.
Our method is different from these methods in that these utilize \hs{prior knowledge from external sources} to better estimate the surrogate model, while we utilize the prior knowledge from \hs{the target source \swp{target source doesn't make sense to me. Is there a more accurate term to use? ``the current task''?} to enhance the training of the \dgdg{target} model}. It means that our method can be applied orthogonally to these methods. 
%In contrast to previous works, the proposed method aims to boost the performance of the BO by further leveraging the knowledge of the network from earlier trials.


\parahead{Self-Distillation}
Knowledge distillation (KD) is a model compression method that involves transferring the knowledge of a large teacher model to a small student model while maintaining performance.
The original work by Hinton et al.~\cite{hinton2015distilling} proposed distilling knowledge by matching the softmax distribution of the teacher and student models.
Since then, various methods have been introduced to improve the knowledge transfer process. For example, FitNets \cite{romero2014fitnets} transfer knowledge by matching outputs from hidden layers of teacher and student models. Attention \cite{zagoruyko2016paying} enforces the student network to mimic the attention maps of the teacher network. Relational
Knowledge Distillation \cite{park2019relational} transfers the mutual relations among data samples via distance-wise and angle-wise distillation loss.

Self-Distillation (SD) is a special form of KD where the teacher and student networks have identical  architecture. 
Born-Again Networks (BAN) \cite{furlanello2018born} demonstrated that when training the student to match the output distribution of the teacher with the identical architecture, it could outperform the teacher. Furthermore, they showed that performing multiple rounds of BAN could further improve the performance where the trained student is set to be a new teacher in the following round.
The effectiveness of SD has been theoretically explained by the \dg{``}multi-view" hypothesis introduced by Allen-Zhu and Li, who showed that self-distillation performs an implicit ensemble of various models \cite{allen2020towards}. Empirical evidence from Pham et al. \cite{pham2022revisiting} suggests that SD encourages the student to find flatter minima, leading to better generalization. In this work, we leverage these observations to improve Bayesian optimization by incorporating the knowledge acquired during intermediate trials through SD.
\swp{In this work, we identify that SD can be an effective method for propagating the task knowledge learned in early stages of BO, to late stages of BO. This combination of the SD and BO processes is key to yielding a high-performing model, which we validate experimentally.}

==> figure/medical.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.45\linewidth,height=0.15\textheight]{figure/breast/LCC(non-cancer).png}
\includegraphics[width=0.45\linewidth,height=0.15\textheight]{figure/nuclei/onco_cpm17_train_Overlay_image_28.png}
\caption{Example images of medical imaging tasks. The image on the left is intended for breast cancer classification, and the image on the right is intended for nuclei instance segmentation.}
\label{fig:example}
\end{center}
\vspace{-5mm}
\end{figure}
